Soft Strategy Selection for Batch-Mode Active Learning

Real-world deployment of active learning typically forces practitioners to choose an acquisition strategy before any data is labeled. This is a daunting task: strategy performance varies widely across settings (e.g. datasets, surrogate models) and cannot be assessed without deployment. Existing strategy selection methods explore one strategy from a portfolio at each round and identify the optimal one using bandit feedback or model retraining. Many acquisition rounds are therefore spent exploring strategies rather than collecting the most informative data. Such overhead is a major barrier to AL-driven design of high-throughput experiments, such as genetic perturbation screens and directed evolution, where AL runs consist of only a few rounds with large batch sizes. This regime permits a natural alternative: acquiring data using multiple AL strategies within a single batch. We refer to this as soft strategy selection and introduce FractAL, a method specifically designed for this task. FractAL infers a per-strategy reward using influence-function-based data attribution, which requires no additional retraining, and then computes budget shares for each strategy in the portfolio using online mirror descent. We benchmark FractAL across 7 setups spanning classification, regression, and genetic perturbation effect prediction. The results highlight that strategy selection is a hard problem: every existing method performs worse than random sampling on at least one setup. FractAL, however, matches or outperforms every baseline, including random sampling, on all 7 setups. Its allocations concentrate budget on the strongest strategies in the portfolio while pruning the weakest. FractAL is therefore a reliable choice for real-world deployments, where the optimal strategy is unknown in advance, an important step towards making AL practical for high-throughput experiments and modern scientific discovery.

==> sections/problem.tex <==
% \subsection{Active Learning Setup}
% We work in a batch mode pool-based active learning setup. For any given task $\mathcal{T}$, we assume access to a large unlabeled pool $\mathcal{D}_{pool}$ and a held-out test set $\mathcal{D}_{test}$ for evaluating the generalization performance of the learner. The learner, also referred to as the surrogate model, is parameterized by $\mathbf{\theta}$ and at any iteration $t$, it is trained on the acquired labeled set $\mathcal{D}^t_L$ using a loss function $\mathcal{L}(\cdot)$. Similar to classic active learning setups, we begin with a pool of data $\mathcal{D}_{start} = \mathcal{D}_{init} \cup \mathcal{D}_{val}$, where $\mathcal{D}_{init}$ is used to warmstart the learner and $\mathcal{D}_{val}$ is used to serve as a proxy for the test set and in model selection. We execute the active learning process to acquire $B$ points per iteration for a total of $N$ iterations, including the initial warmstart iteration.

% \subsection{Adaptive Strategy Mixing}
% We focus on the problem of adaptive strategy mixing for batch active learning and model it as an online convex optimization problem.

% Specifically, let $\mathcal{A} = \{\mathcal{A}_1, \cdots, \mathcal{A}_K\}$ be a set of different data acquisition strategies used commonly in active learning, like Random, CoreSet \citep{sener2017active}, BADGE \citep{ash2019deep} etc. At any iteration $t$, the learner decides an allocation scheme $p^t \in \Delta^{K-1}$ for all the candidates in the pool. The learner then observes a reward $r^t$ for its action. The goal of the learner is to adaptively change allocations to achieve the maximum performance on test set at the end of active learning process. 
\label{sec:prob}
\subsection{Active Learning Framework}
We consider a batch-mode, pool-based active learning (AL) setting. Let $\mathcal{D}_{pool}$ denote a large unlabeled pool and $\mathcal{D}_{test}$ a held-out set for performance evaluation. The learner, a surrogate model $f_\theta$ parameterized by $\theta$, is trained on an evolving labeled set $\mathcal{D}_L^t$ by minimizing a task-specific loss function $\mathcal{L}(\cdot)$. We initialize the process with a seed set $\mathcal{D}_{start} = \mathcal{D}_{init} \cup \mathcal{D}_{val}$, where $\mathcal{D}_{init}$ warmstarts the model and $\mathcal{D}_{val}$ serves as a proxy for the test distribution for model selection and feedback. The AL process proceeds for $N$ iterations, acquiring a batch of $b$ samples at each step $t \in \{1, \dots, N\}$.

\subsection{Adaptive Budget Allocation}
\label{prb:alloc}
We cast the problem of adaptive budget allocation as an online convex optimization task. Given a candidate pool of $K$ acquisition strategies $\mathcal{A} = \{\mathcal{A}_1, \dots, \mathcal{A}_K\}$, the learner must determine an allocation vector $\mathbf{p}^t$ at each iteration $t-1$:
\begin{equation}
    \mathbf{p}^t \in \Delta^{K-1} := \left\{ \mathbf{p} \in [0, 1]^K : \sum_{i=1}^K p_i = 1 \right\}
\end{equation}
where $p^t_i$ represents the fraction of the total budget $b$ assigned to strategy $\mathcal{A}_i$ for acquiring batch $B^t$. This results in a composite acquisition batch $B^t = \bigcup_{i=1}^K B^t_i$, where $|B^t_i| = \lfloor p^t_i * b\rfloor$.

Upon acquiring $B^t$ and updating the model parameters to $\theta^t$, the learner receives a feedback signal $\mathbf{r}^t \in \mathbb{R}^K$. Here, each component $r^t_i$ quantifies the utility or ``reward'' provided by strategy $\mathcal{A}_i$ during that iteration. Our objective is to identify a sequence of allocations $\{\mathbf{p}^t\}_{t=2}^N$ and subsequently $D^N_L = \mathcal{D}_{init} \cup \left(\bigcup\limits_{t=2}^N B^t\right)$\footnote{Since first iteration acquires the warmstart data, $B^1 = \mathcal{D}_{init}$} that maximizes the cumulative performance of the final model:
\begin{equation}
    \max_{\mathbf{p}^2, \dots, \mathbf{p}^N} \mathbb{E} \left[ \text{Perf}(f_{\theta^N}; \mathcal{D}_{test}) \right] 
\end{equation}
where $\text{Perf}(\cdot)$ is the evaluation metric (e.g., accuracy or negative MSE). 
% By optimizing the inner product $\langle \mathbf{p}_t, \mathbf{r}_t \rangle$, we frame the adaptive mixing problem as an online linear optimization task, which we solve via influence-based feedback and mirror descent.

% \approx \max_{\mathbf{p}_1, \dots, \mathbf{p}_N} \sum_{t=1}^N \langle \mathbf{p}_t, \mathbf{r}_t \rangle
